From Newton to Boltzmann: hard spheres and short-range potentials

We provide a rigorous derivation of the Boltzmann equation as the mesoscopic limit of systems of hard spheres, or Newtonian particles interacting via a short-range potential, as the number of particles $N$ goes to infinity and the characteristic length of interaction $\e$ simultaneously goes to $0,$ in the Boltzmann-Grad scaling $N \e^{d-1} \equiv 1.$ The time of validity of the convergence is a fraction of the average time of first collision, due to a limitation of the time on which one can prove uniform estimates for the BBGKY and Boltzmann hierarchies. Our proof relies on the fundamental ideas of Lanford, and the important contributions of King, Cercignani, Illner and Pulvirenti, and Cercignani, Gerasimenko and Petrina. The main novelty here is the detailed study of pathological trajectories involving recollisions, which proves the term-by-term convergence for the correlation series expansion.

==> convergenceproof.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \chapter{Convergence proof}\label{convergenceproof}
\setcounter{equation}{0}
In this chapter we conclude the proof of Theorem~\ref{main-thm} by proving that~$ J^{R,\delta}_{s,n}-  J^{0,R,\delta}_{s,n}$ goes to zero in the Boltzmann-Grad limit, with the notation of the previous chapter, namely~(\ref{boltzmannfunctionalapprox}) and~(\ref{firstbbgkypseudotraj}). 
The main difficulty lies in the fact that in contrast to the Boltzmann situation, collisions in the BBGKY configuration are not pointwise in space, nor in time. At each collision time~$t_k$ a small error is therefore introduced, which needs to be controled.


We recall that, as in the previous chapter, we consider dynamics
\begin{itemize}
\item 
 involving only a finite number $s+n$ of particles, 
 \item with bounded energies (at most $R^2\gg1$), 
 \item   such that the $n$ additional particles are adjoined through binary collisions  at times separated at least by $\delta\ll1$.
 \end{itemize}
 The additional truncation parameters $a,\eps_0,\eta\ll 1$  satisfy (\ref{sizeofparameters}).

 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proximity of Boltzmann and BBGKY trajectories}\label{finalinduction}


This paragraph  is   devoted to the proof, by induction, that the BBGKY and Boltzmann
pseudo-trajectories remain close for all times, in particular that there is no recollision for the BBGKY dynamics. 

We recall that the notation~$Z_k^0(t)$ and~$Z_k(t)$ were defined in Paragraphs~\ref{approxboltzmann}
 and~\ref{approxbbgky}
 respectively.
 \begin{Lem}\label{translation-lem}
Fix $T\in {\mathcal T}_{n,\delta}(t)$, $J$, and~$M$ and given~$Z_s $ in~$ \Delta_s (\eps_0)$, consider  for all $i\in \{1,\dots n\}$, an impact parameter $\nu_{s+i}$ and a velocity~$v_{s+i}$ such that~$(\nu_{s+i},v_{s+i}) \notin {\mathcal B}_{s+i-1}(Z_{s+i-1}^0(t_i))$.
Then, for $\eps$ sufficiently small, for all $i\in [1,n]$, and all $ k\leq s+i$,
\begin{equation}\label{theresult}
| x^\eps_k(t_{i+1}) - x_k^0(t_{i+1}) |   \leq C\eps i
\quad \mbox{and}\quad v_k(t_{i+1 }) = v_k^0(t_{i +1})  \,,
\end{equation}
where the constant $C$ depends only on $\eta, R, \delta$.
\end{Lem}


\begin{proof}
We proceed by induction on~$i$, the index of the time variables~$t_{i+1}$ for~$0\leq i \leq n$. 


We first notice that by construction, $ Z_{s}(t_{1 }) -Z_s^0(t_{1 })=0$, 
so~(\ref{theresult}) holds for~$i=0$. The initial configuration being a good configuration, we indeed know that there is no possible  recollision.



Now let~$i\in [1,n]$ be fixed, and assume that for all~$\ell \leq i$
\begin{equation}\label{theresult2}
\forall k\leq s +\ell-1,\qquad | x^\eps_k(t_{\ell}) - x_k^0(t_{\ell}) |   \leq C\eps (\ell-1)
\quad \mbox{and}\quad v_k(t_{\ell }) = v_k^0(t_{\ell })  \,.
\end{equation}
Let us prove that~(\ref{theresult2}) holds for~$\ell= i+1$.
We shall consider two cases depending on whether the particle adjoined at time~$t_{i}$ is pre-collisional or post-collisional. 

\medskip
\noindent
$\bullet$
As usual, the case of pre-collisional velocities $(v_{s+i}, v_{m_i}(t_i))$ at time $t_i$ is the most simple to handle. We indeed have $\forall \tau \in [t_{i+1},t_i]$
$$ 
\begin{aligned}
&\forall k< s+i\,,\quad x^0_k(\tau) =x^0_k (t_i) +(\tau-t_i) v^0_k(t_i)\,,\qquad v^0_k(\tau) =v^0_k(t_i)\,,\\
&x^0_{s+i}(\tau) = x^0_{m_i} (t_i)  + (\tau-t_i) v_{s+i}\,,\qquad v_{s+i}^0(\tau) =v_{s+i}\,.
\end{aligned}
$$
Now let us study the BBGKY trajectory.
We recall that the particle is adjoined in such a way that~$(\nu_{s+i}, v_{s+i})$  belongs to~$^c{} {\mathcal B}_{s+i-1}  (  Z_{s+i-1}^0(t_i))$. Provided that $\eps$ is sufficiently small, by the induction assumption~(\ref{theresult2}), we have
$$ | X_{s+i-1}^\eps (t_i) -X_{s+i-1}^0 (t_i) |\leq C\eps (i-1) \leq a \,.$$
Since~$Z_{s+i-1}^0(t_i)$ belongs to~$\cG_{s+i-1}(\eps_0)$ (see Paragraph~\ref{approxboltzmann}), we can apply Proposition~\ref{geometric-prop}
which implies  that backwards in time, there is free flow for~$Z^\eps_{s+i}$. In particular,
$$ 
\begin{aligned}
&\forall k< s+i\,,\quad x_k(\tau) =x_k (t_i) +(\tau-t_i) v_k(t_i)\,,\qquad v_k(\tau) =v_k(t_i)\,,\\
&x_{s+i}(\tau) = x_{m_i} (t_i) + \eps \nu_{s+i}  + (\tau-t_i) v_{s+i}\,,\qquad v_{s+i}(\tau) =v_{s+i}\,.
\end{aligned}
$$
We therefore obtain
\begin{equation}\label{induction1}
\forall k\leq s+i\,,\quad \forall \tau \in [t_{i+1},t_i] \, , \quad v_k(\tau ) -v_k^0(\tau) = v_k(t_i ) -v_k^0(t_i) = 0\, ,
\end{equation}
and  
\begin{equation}\label{induction2}\forall k\leq s+i\,,\quad  \forall \tau \in [t_{i+1},t_i] \, , \quad  
 |x_k(\tau)- x_k^0(\tau)| \leq C\eps (i-1) +\eps \,.
 \end{equation}
 
\medskip
\noindent
$\bullet$
The case of post-collisional velocities is a little more complicated since there is a (small) time interval during which  interaction occurs.

Let us start by describing the Boltzmann flow. By definition of the post-collisional configuration, we know that   the following identifies hold: 
$$
\forall t_{i+1} \leq \tau < t_i \, , \quad \left \{\begin{aligned}
 (v_{m_i}^0,v_{s+i}^0 )(\tau) = (v_{m_i}^{0*}(t_i) , v_{s+i} ^* ) \hbox{ with } (\nu_{s+i}^*,v_{m_i}^{0*}(t_i) , v_{s+i} ^* ) := \sigma_0^{-1}( \nu_{s+i}, v_{m_i}^{0}(t_i)  , v_{s+i} ) \\
  x_{m_i}^0 (\tau) = x_{m_i}^0 (t_i) + (\tau - t_i) v_{m_i}^{0*}(t_i) \, ,  \, x_{s+i}^0 (\tau) = x_{s+i}^0 (t_i) + (\tau - t_i) v_{s+i}^{*} \\
 \forall j \notin \{ m_i, s+1\} \,, \quad v_{j}^0(\tau) =v_{j}^0(t_i)  \, , \,  x_j^0(\tau) = x_j^0(t_i) + (\tau - t_i) v_{j}^0(t_i)  \, ,
\end{aligned}
\right.
$$
where~$\sigma_0$ denotes the scattering operator defined in Definition~\ref{scatteringbbgky}
 in Chapter~\ref{scattering}.

First, by Proposition~\ref{geometric-prop}, we know that for $j\notin \{m_i, s+i\}$ and $\forall \tau \in [t_{i+1},t_i]$,
$$ 
 x_j(\tau) =x_j (t_i) +(\tau-t_i) v_j(t_i)\, ,\qquad v_j(\tau) =v_j(t_i)\,,
$$
so that by the induction assumption~(\ref{theresult2}) we obtain
\begin{equation}\label{induction3}
\begin{aligned}
\forall j\notin \{m_i, s+i\} \, , \,  \forall \tau \in [t_{i+1},t_i] \, , \quad  |x_j(\tau)- x_j^0(\tau)| =  |x_j(t_i)- x_j^0(t_i)|  \leq C \eps\\
 \mbox{and} \quad v_j(\tau) =  v^0_j(\tau)\,.
 \end{aligned}
\end{equation}

We now have  to focus on the pair $(s+i, m_i)$. According to Chapter~\ref{scattering}, the relative velocity evolves under the nonlinear dynamics on a  time interval~$[t_i-t_\eps,t_i]$ with $t_\eps \leq C(\eta, R) \eps$ (recalling that by construction, the relative velocity~$|v_{s+i} -  v_{m_i}(t_i)|$ is bounded from above  by $R$ and from below by $\eta$, and that the impact parameter is also bounded from below by $\eta$). Then,    for all $\tau \in [t_{i+1}, t_i-t_\eps ]$,
\begin{equation}\label{thevelocities}
v_{s+i}(\tau) =v_{s+i}^* =  v_{s+i}^0(\tau)  \, , \quad v_{m_i}(\tau) =v_{m_i} ^*(t_i) = v_{m_i}^{0*}(t_i) =v_{m_i}^0  (\tau)  \, .
\end{equation}
In particular,
\begin{equation}\label{induction4}
 v_{s+i}(t_{i+1}) = v_{s+i}^0(t_{i+1}) \quad \mbox{and} \quad  v_{m_i}(t_{i+1})  = v_{m_i}^0(t_{i+1})  \, .
\end{equation}
\noindent
The conservation of total momentum  as in Paragraph \ref{gaindec} shows that
$$
 \begin{aligned}
  \Big|\frac12 (x_{m_i} ^{\eps} (t_i-t_\eps)+x_{s+i} ^{\eps} (t_i-t_\eps)) - \frac12(x_{m_i} ^0 (t_i-t_\eps)+x_{s+i} ^0 (t_i-t_\eps))\Big| \\=\Big|\frac12 (x_{m_i} ^{\eps} (t_i)+x_{s+i} ^{\eps} (t_i) - \frac12(x_{m_i} ^0 (t_i)+x_{s+i} ^0 (t_i))\Big| \\
  = \Big|x_{s+i} ^{\eps} (t_i) - x_{s+i} ^0 (t_i)\Big| +\frac\eps2 \leq C\eps (i-1) +\frac\eps 2 \, \cdotp
 \end{aligned}
 $$
 On the other hand, by definition of the scattering time $t_\eps$, 
 $$
 \begin{aligned}
 |x_{m_i} ^{\eps} (t_i-t_\eps)-x_{s+i} ^{\eps} (t_i-t_\eps)|=\eps \, ,\\
  |x_{m_i} ^0 (t_i-t_\eps)-x_{s+i} ^0 (t_i-t_\eps)| = t_\eps | v_{m_i}^*-v_{s+i}^*|\leq C(\eta, R) \eps \, .
 \end{aligned}
 $$
 We obtain finally
 \begin{equation}\label{outsidescatteringclose}
  |x_{m_i} ^{\eps} (t_i-t_\eps)-x_{m_i} ^0 (t_i-t_\eps)|\leq C\eps i
 \hbox{ and } |x_{s+i} ^{\eps} (t_i-t_\eps)-x_{s+i} ^0 (t_i-t_\eps)| \leq C\eps i
 \end{equation}
  provided that $C$ is chosen sufficiently large (depending on $R$ and $\eta$).
 
 
Now let us apply  Proposition~\ref{geometric-prop}, which implies that
for all $\tau \in [t_{i+1}, t_i-t_\eps]$ the backward in time evolution of the two particles~$x^\eps_{s+i}(t_i-t_\eps )  $ and~$ x^\eps_{m_i} (t_i-t_\eps )  $,  is that of free flow:
 we have therefore, using~(\ref{thevelocities}),
 $$ 
 \begin{aligned}
 x^\eps_{m_i} (t_{i+1})-x^0_{m_i} (t_{i+1})  =x_{m_i}^\eps (t_i-t_\eps ) -x_{m_i}^0  (t_i-t_\eps ) \,,\\
 x^\eps_{s+i} (t_{i+1})-x^0_{s+i} (t_{i+1})  =x_{s+i}^\eps (t_i-t_\eps ) -x_{s+i}^0  (t_i-t_\eps ) \,.
\end{aligned}
$$
From~(\ref{outsidescatteringclose}) we therefore deduce that the induction assumption is  satisfied at time step~$t_{i+1}$, and the proposition is proved.
     \end{proof}
     
     Note that, by construction,
     $$Z_{s+n}^0(0)\in \cG_{s+n}(\eps_0)\,,$$
so that an obvious application of the triangular inequality leads to
 $$Z_{s+n}^\eps(0)\in \cG_{s+n}(\eps_0/2)\,.$$
 Note also that the indicator functions are identically equal to 1 for good configurations.
 We therefore have the following
 
     \begin{Cor}\label{secondbbgkypseudotraj}
    Under the assumptions of Lemma~{\rm\ref{translation-lem}}, the functional~$J^{R,\delta}_{s,n}  (t,J,M)$ defined in~{\rm(\ref{firstbbgkypseudotraj})} may be written as follows:
       $$
\begin{aligned}
   J_{s,n} ^{R,\delta} (t,J,M)(X_s)& = \frac{(N-s)! }{(N- s-n)!}\eps^{n(d-1)} \int_{B_R \setminus \cM_s(X_s)} dV_s \varphi_s(V_s) \int_{{\mathcal T}_{n,\delta}(t)}   dT_n    \\
&\quad \int_{  ^c{} {\mathcal B}_{s}  (  Z_{s}^0(t_1))
}   d\nu_{s+1}  dv_{s+1} \,   (\nu_{s+1}   \cdot ( v_{s+1}  - v_{m_1}(t_1)))_{j_1}    \\ 
 & \quad \dots  \int_{  ^c{} {\mathcal B}_{s+n-1}  (  Z_{s+n-1}^0(t_n))
}  d\nu_{s+n}  dv_{s+n}  \, (\nu_{s+n}   \cdot ( v_{s+n}  - v_{m_n}(t_n)))_{j_n}   \\ 
  &\quad \times  
 \indc_{E_\eps(Z_{s+n}(0))\leq R^2}    \indc_{ Z_{s+n}(0) \in \cG_{s+n}(\eps_0/2)}
  \widetilde f_{N,0}^{(s+n)} (Z^\eps_{s+n}(0))   \, .
\end{aligned}
$$
     \end{Cor}
\section{End of the proof of Theorem~\ref{main-thm}}\label{theend}

The end of the proof of Theorem~\ref{main-thm} consists  in estimating the error terms in~$ J^{R,\delta}_{s,n}-  J^{0,R,\delta}_{s,n}$ coming essentially  from the micro-translations described in the previous paragraph and from the initial data.

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Error coming from  the initial data}$ $
 Let us     replace the initial data in $J^{R,\delta}_{s,n} $ by that of the Boltzmann hierarchy, defining:
 $$
     \begin{aligned}
    \widetilde J^{R,\delta}_{s,n}  (t,J,M)(X_s) &= \frac{(N-s)! }{(N- s-n)!}\eps^{n(d-1)} \int_{B_R \setminus \cM_s(X_s)} dV_s \varphi_s(V_s) \int_{{\mathcal T}_{n,\delta}(t)}   dT_n    \\
&\quad  \int_{  ^c{} {\mathcal B}_{s}  (  Z_{s}^0(t_1))
}  \!  \!  \!  \!  \!  d\nu_{s+1}  dv_{s+1} \,   (\nu_{s+1}   \cdot ( v_{s+1}  - v_{m_1}(t_1)) )_{j_1}  \\
 &\qquad   \dots  \int_{  ^c{} {\mathcal B}_{s+n-1}  (  Z_{s+n-1}^0(t_n))
}  \!  \!  \!  \!  \!  d\nu_{s+n}  dv_{s+n}  \, (\nu_{s+n}   \cdot ( v_{s+n}  - v_{m_n}(t_n)))_{j_n}   \\ 
 & \qquad \times    \indc_{E_0(Z_{s+n}(0))\leq R^2}   \indc_{ Z^\eps_{s+n}(0) \in \cG_{s+n}(\eps_0/2)}        f_{0}^{(s+n)} (Z_{s+n}(0))   \, .
\end{aligned}
   $$

   
    \begin{Lem}\label{data}
In the Boltzmann-Grad scaling $N \eps^{d-1} = 1$,
$$
  \big |  \1_{\Delta^X_s (\eps_0)} (J^{R,\delta}_{s,n}-  \widetilde J^{R,\delta}_{s,n} )  (t,J,M)(X_s) \big | \leq  C{R^{dn} T^n\over n!} \| \varphi_s\| _{L^\infty(\R^{ds})} \big\|  \1_{\Delta_{s+n} (\eps_0/2)} (  \widetilde f^{(s+n)}_{N,0}   - f^{(s+n)}_{0}) \big \| _{L^\infty(\R^{2d(s+n)})}
$$
 and in particular
$$
 |  \1_{\Delta^X_s (\eps_0)} (\widetilde I_{s,n}-  \widetilde J_{s,n} )  (t,J,M)(X_s)  | \to 0 \hbox{ as } \eps \to 0  \, ,
$$
 uniformly in $t\in [0,T]$ and $X_s\in \R^{ds}$.
\end{Lem}
\begin{proof}
We recall that by assumption,  $ \1_{\Delta_{s+n} (\eps_0/2)} (  \widetilde f^{(s+n)}_{N,0}   - f^{(s+n)}_{0}) $ goes to zero uniformy in~$Z_{s+n}$.
 
 
 By definition of the good sets~${\mathcal G}_k(c)$, the positions in the argument of~$   \widetilde f^{(s+n)}_{N,0} -  f^{(s+n)}_{0}$ satisfy the separation condition~$|x_{i} - x_j | \geq \eps_0/2$ for~$i \neq j$~:
$$\indc_{{\mathcal G}_{s+n}(\eps_0/2)}    (  \widetilde f^{(s+n)}_{N,0}   - f^{(s+n)}_{0}) =\indc_{{\mathcal G}_{s+n}(\eps_0/2)}  \indc_{\Delta_{s+n}(\eps_0/2)}    (  \widetilde f^{(s+n)}_{N,0}   - f^{(s+n)}_{0}) \,.$$
Furthermore, due to that   separation condition,
$$ E_\eps(Z_{s+n}) =E_0(Z_{s+n}) =\frac12 \sum_{i=1}^{s+n} |v_i|^2\,.$$
So we can write
$$
     \begin{aligned}
      (J^{R,\delta}_{s,n}(t,J,M)-  \widetilde J^{R,\delta}_{s,n}(t,J,M))(X_s) & = \frac{(N-s)! }{(N- s-n)!}\eps^{n(d-1)} \int_{B_R \setminus \cM_s(X_s)} \! \! \!  dV_s \varphi_s(V_s) \int_{\mathcal T_{n,\delta}(t)}   dT_n  \\
     &\quad    \int_{  ^c{} {\mathcal B}_{s}  (  Z_{s}^0(t_1))
}   d\nu_{s+1}  dv_{s+1}   (\nu_{s+1}   \cdot ( v_{s+1}  - v_{m_1}(t_1))  )_{j_1}  
  \\ &\qquad \dots  \int_{  ^c{} {\mathcal B}_{s+n-1}  (  Z_{s+n-1}^0(t_n))
}   d\nu_{s+n}  dv_{s+n}  \, (\nu_{s+n}   \cdot ( v_{s+n}  - v_{m_n}(t_n)) )_{j_n}  \\ 
    &\qquad    \times   \indc_{E_\eps(Z^\eps_{s+n}(0))\leq R^2} \indc_{\Delta_{s+n}(\eps_0/2)}    ( \widetilde f^{(s+n)}_{N,0} -f^{(s+n)}_0 )   \, ,\end{aligned}
   $$
and
 we find directly that
 $$
     \begin{aligned}
  & \Big| \1_{\Delta^X_s(\eps_0)}(J^{R,\delta}_{s,n}(t,J,M)-  \widetilde J^{R,\delta}_{s,n}(t,J,M))(X_s)\Big|    \\
  &\quad \leq C{R^{dn} T^n\over n!} \| \varphi_s\| _{L^\infty(\R^{ds})} \big\|  \1_{\Delta_{s+n}(\eps_0/2)} (  \widetilde f^{(s+n)}_{N,0}   - f^{(s+n)}_{0}) \big \| _{L^\infty(\R^{2d(s+n)})} \, .
 \end{aligned}
  $$
   The result is proved.\end{proof}

\subsection{Error coming from the prefactors in the collision operators}$ $
As $\eps \to 0$ in the Boltzmann-Grad scaling, we have 
$$
 \frac{(N-s)! }{(N- s-n)!}\eps^{n(d-1)} \to 1 \, .
$$
Defining
\begin{equation}
\label{lastfunctional}
     \begin{aligned}
   \overline J^{R,\delta}_{s,n}  (t,J,M)(X_s) &= \int_{B_R \setminus \cM_s(X_s)} dV_s \varphi_s(V_s) \int_{{\mathcal T}_{n,\delta}(t)}   dT_n\\
   &\quad   \int_{  ^c{} {\mathcal B}_{s}  (  Z_{s}^0(t_1))
}   d\nu_{s+1}  dv_{s+1} \,  ( \nu_{s+1}   \cdot ( v_{s+1}  - v_{m_1}(t_1)))_{j_1}    \\ 
 & \qquad  \dots  \int_{  ^c{} {\mathcal B}_{s+n-1}  (  Z_{s+n-1}^0(t_n))
}  d\nu_{s+n}  dv_{s+n}  \, (\nu_{s+n}   \cdot ( v_{s+n}  - v_{m_n}(t_n)) )_{j_n}  \\ 
  & \qquad \times    \indc_{E_0(Z_{s+n}(0))\leq R^2}   \indc_{ Z^\eps_{s+n}(0) \in \cG_{s+n}(\eps_0/2)}        f_{0}^{(s+n)} (Z_{s+n}(0))   \, ,
\end{aligned}
\end{equation}
   we have the following obvious convergence.   
    \begin{Lem}\label{cross-section}
In the Boltzmann-Grad scaling $N \eps^{d-1} = 1$,
$$
  |  \1_{\Delta^X_s} (\widetilde J^{R,\delta}_{s,n}-\overline  J^{R,\delta}_{s,n}  ) (t,J,M)(X_s) |\leq  C{ s(s+n) \over N} \|\varphi\|_{L^\infty (\R^{ds})}
  \Nt{  F_{N,0}}_{0,\beta_0,\mu_0}\,.
$$
\end{Lem}

\subsection{Conclusion} We can now compare the definition (\ref{boltzmannfunctionalapprox}) of $J^{0,R,\delta}_{s,n}  (t,J,M)$ 
$$  \begin{aligned}
     J^{0,R,\delta}_{s,n} (t,J,M)(X_s)&   =  \int_{B_R \setminus \cM_s(X_s)} dV_s  \varphi_s(V_s) 
     \int_{{\mathcal T}_{n,\delta}(t)}  dT_n\\
 &\quad  \int_{^c{} {\mathcal B}_{s} (  Z_s^0(t_1))} \!  \!  \!  \!  \!  d\nu_{s+1} dv_{s+1}
  ((v_{s+1} - v_{m_1}^0(t_1)\cdot \nu_{s+1} )_{j_1} \\
       &\qquad\dots    \int_{^c{} {\mathcal B}_{s+n-1}i (  Z_{s+n-1}^0(t_n))}   \!  \!  \!  \!  \! d\nu_{s+n} dv_{s+n}
  ((v_{s+n} - v_{m_n}^0(t_n)\cdot \nu_{s+n} )_{j_n} \\
  & \qquad  \indc_{E_0(Z_{s+n}^0 (0))\leq R^2}    f^{(s+n)}_{0}   (Z_{s+n}^0 (0))  \, .
   \end{aligned}
$$
and the formulation (\ref{lastfunctional}) for the approximate BBGKY hierarchy
$$   \begin{aligned}
   \overline J^{R,\delta}_{s,n}  (t,J,M)(X_s) &= \int_{B_R \setminus \cM_s(X_s)} dV_s \varphi_s(V_s) \int_{{\mathcal T}_{n,\delta}(t)}   dT_n\\
   &\quad   \int_{  ^c{} {\mathcal B}_{s}  (  Z_{s}^0(t_1))
}   d\nu_{s+1}  dv_{s+1} \,  ( \nu_{s+1}   \cdot ( v_{s+1}  - v_{m_1}(t_1)))_{j_1}    \\ 
 & \qquad \dots  \int_{  ^c{} {\mathcal B}_{s+n-1}  (  Z_{s+n-1}^0(t_n))
}  d\nu_{s+n}  dv_{s+n}  \, (\nu_{s+n}   \cdot ( v_{s+n}  - v_{m_n}(t_n)) )_{j_n}  \\ 
  & \qquad \times    \indc_{E_0(Z_{s+n}(0))\leq R^2}   \indc_{ Z^\eps_{s+n}(0) \in \cG_{s+n}(\eps_0/2)}        f_{0}^{(s+n)} (Z_{s+n}(0))   \, .
\end{aligned}
$$


 Lemma \ref{translation-lem} implies  that at time~$0$
we have
$$ | X_{s+n}(0 )- X_{s+n}^0(0)| \leq C(R,\eta) n \eps\, ,\quad \mbox{and} \quad  V_{s+n}(0 )= V_{s+n}^0(0)\, .$$

Provided that $f_0^{(s+n)}$ is continuous, we then obtain the expected convergence and  this concludes the proof of Theorem~\ref{main-thm}.  

Notice for instance that if $f_0^{(s+n)}$ is Lipschitz, then we have the following estimate.
\begin{prop}
In the Boltzmann-Grad scaling $N \eps^{d-1} = 1$,
$$
  |  \1_{\Delta^X_s(\eps_0)} (I^0-\overline  J  )  (t,X_s)  | \leq C(R,\eta) n \eps \| \nabla_{X_{s+n}} f_0^{(s+n)} \|_{L^\infty}\,,
$$
 uniformly in $t\in [0,T]$ and $X_s\in \R^{ds}$.

\end{prop}
   

==> geometry.tex <==
\chapter{Elimination of recollisions}\label{pseudotraj}
\setcounter{equation}{0}
We have seen in the previous chapter that the convergence of observables (stated in Theorem~\ref{main-thm} in Chapter~\ref{convergenceresult}) reduces to the convergence to zero of the functional~$I_{s,n}^{R,\delta} -I_{s,n}^{0,R,\delta}  $, defined in~(\ref{defIsnRdelta}), corresponding to  dynamics
\begin{itemize}
\item 
 involving only a finite number $s+n$ of particles, 
 \item with bounded energies (at most $R^2$), 
 \item   such that the $n$ additional particles are adjoined through binary collisions, 
 \item at times separated at least by $\delta$.
 \end{itemize}
 
 \bigskip
 
% 
% To make notation lighter in the following we shall {\em systematically omit to specify that energies are bounded by~$R^2$}: we shall always assume collision operators act on energy-truncated functions at~$R^2$, and due to Remark~\ref{colltrunccommute}, the energy after collision remains truncated at~$R^2$.
 
  

 
 
 Let us denote, for any constant~$c>0$, by\label{indexdefGk} $\cG_k(c)$ the set of ``good configurations" of $k$ particles, separated by at least~$c$ through backwards transport: that is
 the set of  $(X_k,V_k) \in \R^{dk} \times B_R^k$ such that
 the image of $(X_k, V_k)$ by the backward free transport satisfies the separation condition
 $$\forall \tau\geq 0 ,\quad \forall i\neq j ,\quad  |x_i-x_j-\tau(v_i-v_j)| \geq c\,,$$
 in particular it  is never collisional.
  We recall that~$ B_R^k := \Big\{V_k \in \R^{dk} \, / \, |V_k| \leq R\Big\}$ and in the following we write~$B_R:=B_R^1$.


 Our goal in the present chapter is to slightly modify (in a uniform way) the  functionals~$I_{s,n}^{R,\delta} $ and~$I_{s,n}^{0,R,\delta} $ in order for the corresponding BBGKY pseudo-trajectories to be decomposed as a succession of free transport and binary collisions, without any recollision. Paragraph~\ref{proposition-geometry} is devoted to the statement and the proof of a geometrical proposition showing how to eliminate bad sets in phase space so that for any particle outside such bad sets, adjoined to a 
 good configuration, the resulting configuration is again  a good configuration. This is applied to the Boltzmann and BBGKY hierarchies in Paragraph~\ref{truncationBB}.
 
 
\section{Elimination of bad sets in phase space leading to recollisions}\label{proposition-geometry}
\setcounter{equation}{0}
\subsection{Statement of the result}
In this section we momentarily forget the BBGKY and Boltzmann hierarchies, and focus on the study of  pseudo-trajectories. More precisely 
our aim is to show that ``good configurations" are stable by adjunction of a collisional particle provided that the deflection angle and the velocity of the additional particle do not belong to a small pathological set. Furthermore the set to be excluded can be chosen in a uniform way with respect to the initial positions of the particles in a small neighborhood of any fixed ``good configuration".

 
\begin{nota} \label{ssmall} In all the sequel, given two parameters $\eta_1$ and $\eta_2$, we shall say that  $$\eta_1 \ll \eta_2 \,  \hbox{ if } \,\eta_1 \leq C \eta_2$$
for some large constant $C$ which does not depend  on any parameter.\end{nota}




\begin{prop}\label{geometric-prop}
Let $ a,\eps_0,\eta\ll 1$  be  such that
\begin{equation}\label{sizeofparameters}
 a \ll \eps_0 \ll \eta \delta \, .
\end{equation}
 Given~$\overline Z_k \in \cG_k(\eps_0)$, there is a subset~$\cB_k(\overline Z_k)$ of~${\mathbf S}_1^{d-1} \times B_R$  of small measure
\begin{equation}
\label{pathological-size}
\big |\cB_k(\overline Z_k) \big |  \leq C(R) \eta^{d-1} + C(R,\Phi,\eta) \Big(
  \frac{a}{\eps_0} +  \frac{\eps_0}{\delta} 
\Big)^{d-1}  \, , 
\end{equation}
and  such that good configurations close to $\overline Z_k$  are stable by adjunction of a collisional particle close to~$\bar x_k$ and not belonging to $\cB_k(\overline Z_k)$, in the following sense. 

Consider~$(\nu,v) \in ({\mathbf S}_1^{d-1} \times B_R) \setminus  \cB_k(\overline Z_k)$ and let~$Z_k$ be a configuration of $k$ particles such that~$V_k = \overline V_k$ and~$
| X_k- \overline X_k  | \leq a $. 

$ \bullet $ $ $ If~$\nu \cdot (v-\bar v_k)< 0$ then for all~$\eps > 0$ sufficiently small,
\begin{equation}\label{taugeq0precoll}
\forall \tau \geq 0 \, , \quad \left\{ \begin{aligned}
\forall i \neq j \in [1,k] \, , \quad  |  (x_i - \tau \bar v_i) - (x_j - \tau \bar v_j ) | \geq \eps \, ,\\
\forall j \in [1,k] \, , \quad |  (x_k + \eps \nu - \tau v) - (x_j - \tau \bar v_j ) | \geq \eps \, .
\end{aligned}
\right.
\end{equation}
Moreover after the time~$\delta$, the~$k+1$ particles are in a good configuration:
\begin{equation}\label{taugeqdelta2precoll}
(X_k - \delta \overline V_k   ,\overline V_k , x_k + \eps \nu - \delta v , v) \in \cG_{k+1} (\eps_0/2)\, .
\end{equation}

$ \bullet $ $ $ If~$\nu \cdot (v-\bar v_k)> 0$ then define for~$j \in [1,k-1]$
$$
(z_k^{\eps*},z^{\eps*}):=\sigma_\eps^{-1} \big (z_k,(x_k + \eps \nu , v) \big) \quad \mbox{and} \quad z_j^{\eps*}:=(x_j-t_\eps \bar v_j, \bar v_j) \, ,$$
 where~$\sigma_\eps$ is
the scattering operator  as  in Definition~{\rm\ref{scatteringbbgky}} and where~$t_\eps$ denotes the scattering time between~$z_k$ and~$(x_k + \eps \nu , v)$.
Then  for all~$\eps > 0$ sufficiently small,
\begin{equation}\label{taugeq0postcoll}
\forall \tau \geq 0 \, , \quad
\left\{ \begin{aligned}
\forall i \neq j \in [1,k ] \, , \quad   |  (x_i^{\eps*}  - \tau v_i^{\eps*} ) - (x_j^{\eps*}  - \tau v_j^{\eps*} ) | \geq \eps \, ,\\
\forall j \in [1,k] \, , \quad  |   ( x^{\eps*}   - \tau  v^{\eps*} ) - (x_j^{\eps*}  - \tau v_j^{\eps*} )| \geq \eps \, .
\end{aligned}\right.\end{equation}
Moreover after the time~$\delta$, the~$k+1$ particles are in a good configuration:
\begin{equation}\label{taugeqdelta2postcoll}
\Big(X_k^{\eps*} -(\delta  -t_\eps) V_k^{\eps*}   ,  V_k^{\eps*}   , x^{\eps*}    -  (\delta  -t_\eps)  v^{\eps*}  , v^{\eps*} \Big) \in \cG_{k+1}(\eps_0/2) \, .
\end{equation}
\end{prop}
The proof of the proposition may be found in Section~\ref{proofgeometric-prop}. It relies on two elementary geometrical lemmas, stated and proved in the next section. The first one describes the bad trajectories associated to the (free) transport. The second one explains how they are modified by the scattering.

\begin{Rem}\label{betterresult}
For the sake of simplicity, we have assumed that the additional particle collides with the particle $k$. Of course, a simple symmetry argument shows that an analogous statement holds if the particle $k+1$ is added close to any of the particles in $Z_k$.

The proof of Proposition~{\rm\ref{geometric-prop}} shows that if~$Z_k = \overline Z_k$ then the factor~$\eps_0/2$ in~{\rm(\ref{taugeqdelta2precoll})} and~{\rm(\ref{taugeqdelta2postcoll})}  may be replaced by~$\eps_0$. The loss comes from the fact that the set to be excluded has to be chosen in a uniform way with respect to the initial positions of the particles in a small neighborhood of $\bar X_k$.

\end{Rem}

\subsection{Two geometrical lemmas}\label{geometry}
%\setcounter{equation}{0}

In this section we state and prove two geometrical lemmas which though elementary, are the key to the proof of Proposition~\ref{geometric-prop}.
   Here and in   the sequel, we   denote by~$K(y,\rho)$\label{defindexKyeta} the cylinder of axis $y\in \R^d$ and radius $\rho>0$ and by~$B_{\rho}(y)$ the ball centered at~$y$ of radius~$\rho$.
 
   \begin{Lem}\label{geometric-lem1}
 Given~$ \bar a>0$ satisfying~$\eps \ll \bar  a \ll \eps_0 $,
   consider $\bar x_1,\bar x_2$ in~$\R^d$ such that $| \bar x_1-\bar x_2|\geq \eps_0$,  and~$ v_1 \in B_R$.
 Then for any~$x_1 \in B_{\bar a}(\bar x_1 )$, any~$x_2 \in B_{\bar a}(\bar x_2 )$  and any $ v_2\in B_R$, the following results hold.
 
 $ \bullet $ $ $ If   $v_1 -v_2 \notin K(\bar x_1-\bar x_2, 6 R\bar a /\eps_0)$, then
  $$
   \forall \tau\geq 0 \,, \quad |(x_1-v_1 \tau)-(  x _2-v_2\tau)| >\eps \, ;
   $$
 $ \bullet $ $ $ If  ~$v_1 -v_2 \notin K(\bar x_1-\bar x_2, 6 R\eps_0/\delta)$
   $$
   \forall \tau\geq \delta  \,, \quad |(x_1-v_1 \tau)-(  x _2-v_2\tau)| >\eps_0 \, .
 $$
 \end{Lem}
 
 
   \begin{proof}
    $ \bullet $ $ $Assume that there exists $\tau_*$ such that
$$ |(x_1-v_1 \tau)-(  x _2-v_2\tau) |\leq \eps\,.$$
Then, by the triangular inequality and provided that $\eps$ is sufficiently small,
$$
|(\bar x_1 -\bar x_2) -  \tau_*(v_1 -v_2)| \leq    \eps+2\bar a \leq 3\bar a \,.
 $$
This means that $( v_1 -v_2)$ belongs to the cone of vertex 0 based on the ball centered at~$\bar x_1 -\bar x_2$ and of radius $  3\bar a $,   which is a cone of solid angle $( 3\bar a /|\bar x_1 -\bar x_2|)^{d-1}$ (since $\bar a \ll \eps_0$).

The intersection of this  cone and of the sphere of radius $2R$  is obviously embedded in the cylinder of axis $\bar x_1 -\bar x_2$ and radius $6R\bar a /\eps_0$, which proves the first result.

 $ \bullet $ $ $ Similarly   assume that there exists $\tau^* \geq \delta $ such that
$$|(x_1-v_1 \tau)-(  x _2-v_2\tau) |\leq \eps_0 \,.$$
Then, by the triangular inequality again,
$$|(\bar x_1 -\bar x_2) -  \tau_*(v_1 -v_2) |\leq \eps_0+2\bar a    \leq 3  \eps_0 \,.$$
In particular, for any unit vector $n$ orthogonal to $\bar x_0-\bar x$,
$$\tau^* | n\cdot (v_1-v_2) |=|n\cdot \left( (\bar x_1 -\bar x_2) -  \tau_*(v_1 -v_2)\right) |   \leq 3 \eps_0 \, .$$
This  tells us exactly  that $v_1-v_2$ belongs to the cylinder of axis $\bar x_1 -\bar x_2$ and radius $3\eps_0/\delta$.
 
 The lemma is proved.
\end{proof}


 The second   geometrical lemma   requires the use of notation coming from scattering theory, introduced in Chapter~\ref{scattering}: it states that if two points~$z_1, z_2 $ in~$ \R^{2d}$ are in a post-collisional configuration and if~$v_1$ or~$v_2$ belong to a cylinder as in Lemma~\ref{geometric-lem1}, then the pre-image $z_2^*$ of~$z_2$ through the scattering operator belongs to a small set of~$\R^{2d}$.
 
 \begin{Lem}\label{geometric-lem3}
Consider  two parameters $\rho\ll R$  and~$\eta \ll 1$, and $(y,w) \in \R^d \times B_R$. 
For any~$v_1 $ in~$ B_R$, define  
$$
\begin{aligned}
\cN^*( y,w,\rho) (v_1) :=\big\{ (\nu ,v_2 )\in {\mathbf S}_1^{d-1}\times  B_R  \,/\, & (v_2-v_1) \cdot \nu > \eta \, ,  \\
&   v^*_1\in w+K(y,\rho) \hbox{ or }  v^*_2 \in w+K(y,\rho) \big\}\, ,
\end{aligned}
$$
where~$(\nu^*, v^*_1, v_2^*)=\sigma_0^{-1}(\nu,v_1,v_2)$ with the notations of Chapter~{\rm\ref{scattering}}.
Then
$$|\cN^*( y,w,\rho) (v_1) | \leq C (\Phi,R,\eta)  \rho^{d-1} $$
where the constant  depends on $\Phi$ through the $L^\infty$ norm of the cross-section $b$ defined in Chapter~{\rm\ref{scattering}}.
\end{Lem}
  




\begin{proof} 
Denote by 
$r =|v_1-v_2|=|v_1^*-v_2^*|$, and by $\omega$ the deflection angle.
The formula (\ref{scattering-def1}) shows that, as $\omega$ varies in ${\mathbf S}_1^{d-1}$, $v^*_1$ and $v^*_2$ range over a sphere of diameter $r$.






The solid angle of the intersection of such a  sphere with the cylinder $w+ K(y,\rho)$  is less than 
$$C_d \min\left(1, \left( {\rho\over r}\right)^{d-1}\right) $$
which implies that 
$$
\begin{aligned}
\left| \{ (\omega, v_2) \,/\,  v_1^*\in w+K(y,\rho) \hbox{ or }  v_2^* \in w+K(y,\rho)\} \right| &\leq C_d \int r^{d-1} \min \left(1, \left( {\rho\over r}\right)^{d-1}\right) dr\\
& \leq C_d R \rho^{d-1} 
\end{aligned}
$$
According to Chapter~\ref{scattering}, the change of variables
$ (\nu,v_1-v_2) \mapsto  (\omega,v_1- v_2)$
is a Lipschitz diffeomorphism away from $\nu \cdot (v_1-v_2) = 0.$ We therefore get the expected estimate.
 \end{proof}
\begin{Rem}
Note that those two lemmas  consist in eliminating  sets in the  velocity variables and deflection angles only, and do not concern the position variables.
\end{Rem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Proposition \ref{geometric-prop}}\label{proofgeometric-prop} 
  We fix a good configuration~$\overline Z_k \in \cG_k(\eps_0)$, and we consider a configuration~$ Z_k \in \R^{2dk}$, with the same velocities as~$\overline Z_k$, and neighboring positions: $| X_k - \overline X_k | \leq a$. In particular we notice that
  for all~$ \tau\geq 0 $ and all~$ i\neq j$,
 \begin{equation}\label{almostgood}
  |x_i-x_j-\tau(\bar v_i-\bar v_j)| \geq  | \bar x_i-\bar x_j-\tau(\bar v_i-\bar v_j)| - 2a \geq \eps_0 /2
  \end{equation}
   since~$a \ll \eps_0$. This implies that~$ Z_k \in \cG_k(\eps_0/2)$.
   Next we consider an additional particle $(x_k+\eps \nu,v_{k+1})$  and we shall separate the analysis into two parts, depending on whether the situation is pre-collisional (meaning~$  \nu \cdot (v_{k+1}-\bar v_k) < 0$) or post-collisional (meaning~$  \nu \cdot (v_{k+1}-\bar v_k) >0$).


 \subsubsection{The pre-collisional case}\label{decloss}
We assume that
 $$  \nu \cdot (v_{k+1}-\bar v_k) < 0\,,$$
meaning that~$(x_k + \eps\nu,v)$ and~$z_k$ form a pre-collisional pair. In particular we have for all times~$\tau \geq 0$ and all~$\eps >0$
$$
\big | \big (
x_k+\eps \nu - v _{k+1}\tau
\big) - \big(
x_k - \bar v_k \tau
\big) \big | \geq \eps \, .
$$
Furthermore up to excluding the ball~$B_\eta(\bar v_k)$ in the set of admissible~$v_{k+1}$, we may assume that
$$
|v_{k+1}-\bar v_k| > \eta \, .
$$
Under that assumption we have for all~$\tau \geq \delta$ and all~$\eps>0$ sufficiently small,
$$
\begin{aligned}
\big | \big (
x_k+\eps \nu - v _{k+1}\tau
\big) - \big(
x_k - \bar v_k \tau
\big) \big | & \geq \tau |v_{k+1}- \bar v_k| - \eps \\
& \geq  {\delta  }\eta- \eps > \eps_0/2 \, . 
\end{aligned}
$$
Furthermore we know that~$Z_{k }$ belongs to~$\cG_{k }(\eps_0/2)$ thanks to~(\ref{almostgood}).  

\noindent Now let~$j \in [1,k-1]$ be given.  According to Lemma~\ref{geometric-lem1}, we
find that
for any $v_{k+1}  $ belonging to the set~$ B_R \setminus K(\bar x_j-\bar x_k, 6 Ra /\eps_0+6 R\eps_0/\delta) ,$
we have
$$ \forall \tau \geq0 \, , \quad |(x_{k }+ \eps \nu-v _{k+1} \tau)-(x_j-\bar v_j \tau)| >\eps \,,$$
and
$$ \forall \tau \geq \delta \, , \quad |(x_{k }+ \eps \nu-v_{k+1}  \tau)-(x_j-\bar v_j \tau)| >\eps_0 \,.$$
Notice that
 $$
 \Big|B_R \cap K(\bar x_j-\bar x_k, 6 Ra /\eps_0+6 R\eps_0/\delta)  \Big|  \leq  C (R) \left({a\over\eps_0}+{\eps_0\over \delta}\right)^{d-1}\, .
 $$
Defining~$\displaystyle \cM^{-} (\overline Z_k):= \bigcup_{j \leq k-1} K(\bar x_j-\bar x_k, 6 Ra /\eps_0+6 R\eps_0/\delta)  $ and
$$
{\mathcal B}_k^-(\overline Z_k):= {\mathbf S}_1 ^{d-1} \times \Big(B_\eta(\bar v_k) \cup\cM^{-} (\overline Z_k)\Big)
$$
we find that
$$
\Big |{\mathcal B}_k^-(\overline Z_k) \Big | \leq   C (R) \Big(\eta^d + \big({a\over\eps_0} \big)^{d-1} + \big({\eps_0\over\delta} \big)^{d-1}\Big)
$$
and~(\ref{taugeq0precoll}) and~(\ref{taugeqdelta2precoll}) hold as soon as~$(\nu,v_{k+1} ) \notin {\mathcal B}_k^-(\overline Z_k)$.
 
  
   \subsubsection{The post-collisional case}\label{gaindec}
We now assume that
 $$  \nu \cdot (v_{k+1} -\bar v_k) > 0\,.$$
 Next let us define
  \begin{equation}\label{defcone}
 C(\overline Z_k):=\Big \{(\nu,v_{k+1} ) \in {\mathbf S}_{1}^d \times B_R \, , \,  \nu \cdot (v_{k+1} - \bar v_k)  \leq \eta  \Big\} \, ,
 \end{equation}
 which satisfies
 $$
 |C(\overline Z_k)| \leq C(R) \eta^{d-1}\,  . 
 $$
 Choosing~$(\nu,v_{k+1} ) \in  ({\mathbf S}_{1}^d \times B_R) \setminus C(\overline Z_k)$   ensures that the cross-section is well defined (see Definition~\ref{def:b}), and that the scattering time~$t_\eps$ is  of order $C(R,\eta)\eps$ by Proposition~\ref{scatteringestimates}.
   
  Considering the formulas~(\ref{scattering-def1})
expressing~$(z^{\eps*}_{k},z^{\eps*}_{k+1} )$ in terms of~$\big(z_k,(x_{k }+\eps \nu, v_{k+1} )\big )$, we know    that
\begin{equation}\label{distancex*x}
|x_k - x_k^{\eps*}|    \leq   \eps + R t_\eps \leq C(R,\eta) \eps \quad \mbox{and} \quad  |(x_{k }+\eps \nu)- x^{\eps*}_{k+1} |  \leq   \eps  +R t_\eps   \leq C(R,\eta) \eps\, .
\end{equation}
 Note that due to~(\ref{almostgood}), all particles $x_j$ with $j\leq k-1$ are at a distance at least $\eps_0/2-\eps\gg \eps$ of the particles $x_k$ and~$ x_{k }+\eps \nu $. Since  they have bounded velocities, they cannot enter the protection spheres of these post-collisional particles  during the interaction time $t_\eps$, provided that $\eps$ is small enough:
 $$R t_\eps \ll \eps_0.$$
   Since the dynamics of the particles $j \leq k-1$ is not affected by the scattering, we get    that~$Z_{k-1}^{\eps*}$  
belongs to~${\mathcal G}_{k-1}(\eps_0/2)$: 
\begin{equation}\label{k-1good}
  \forall \tau\geq 0 \, , \, \forall (i,j) \in [1, k-1] ^2\hbox{ with } i\neq j \, ,\quad  |x_i^{\eps*} -x_j^{\eps*} -\tau(v_i^{\eps*} -v_j^{\eps*} )| \geq \eps_0/2\,. 
  \end{equation}


  
The pair~$(z_k^{\eps*},z^{\eps*}_{k+1})$ is a pre-collisional pair by definition, so we know that for all~$\tau \geq 0$,
$$
 |  (x_k^{\eps*}  - \tau v_k^{\eps*} ) - ( x^{\eps*}_{k+1}   - \tau  v_{k+1}^{\eps*} ) | \geq \eps \, .
$$
Moreover we have $|v^{\eps*}_k-v^{\eps*}| = |\bar v_k-v_{k+1}|> \eta$, so as in the pre-collisional case above we have
  $$ \forall \tau\geq \delta \, , \quad  |x_k^{\eps*}-x^{\eps*}-\tau(v_k^{\eps*}-v_{k+1}^{\eps*})| \geq \eta \delta - \e \geq   \eps_0 \,,
 $$
 for $\eps$ sufficiently small, since~$ \eps_0 \ll  \eta \delta$.
 

 Next for~$j \leq k-1$ we have for $\eps$ sufficiently small, recalling that the uniform, rectilinear motion of the center of mass as described in~(\ref{rectiunif}),
  $$
 \begin{aligned}
  | x_j ^{\eps*} - \bar x_j| \leq  | x_j ^{\eps*} -   x_j|  + | x_j   - \bar x_j| \leq Rt_\eps + a \leq 2a \\
  | x_k ^{\eps*} - \bar x_k| \leq  \frac12 | x_k ^{\eps*} -   x_{k+1}^{\eps^*}|  + \frac12 |(x_k ^{\eps*} +   x_{k+1}^{\eps^*})-(x_k+x_{k+1})|+\frac12  |(x_k+x_{k+1})   - 2\bar x_k|\\ \leq Rt_\eps +\eps  + a \leq 2a \\
 | x_{k+1} ^{\eps*} - \bar x_k| \leq  \frac12 | x_k ^{\eps*} -   x_{k+1}^{\eps^*}|  + \frac12 |(x_k ^{\eps*} +   x_{k+1}^{\eps^*})-(x_k+x_{k+1})|+\frac12  |(x_k+x_{k+1})   - 2\bar x_k|\\
  \leq Rt_\eps +\eps  + a \leq 2a\, .
 \end{aligned}
 $$
By Lemma \ref{geometric-lem1}, provided  $v_k^{\eps*}$ and~$v_{k+1}^{\eps*} $ do not belong to
$$ \bar v_j+K(\bar x_j -\bar x_k, 12Ra/\eps_0+12R\eps_0/\delta) \cap B_R \, , 
$$
we get since~$v_j^{\eps*}  = \bar v_j$,
$$\begin{aligned}
  \forall \tau\geq 0 \, , \quad  |x_k^{\eps*}-x_j^{\eps*}-\tau(v_k^{\eps*}-v_j^{\eps*})| &\geq  \eps\,,\\
 \mbox{and}\quad  |x^{\eps*}-x_j^{\eps*}-\tau(v_{k+1}^{\eps*}-v_j^{\eps*})| &\geq \eps
 \end{aligned}  $$
as well as
$$\begin{aligned}
  \forall \tau\geq \delta/2 \, , \quad  |x_k^{\eps*}-x_j^{\eps*}-\tau(v_k^{\eps*}-v_j^{\eps*})| &\geq  \eps_0/2\,,\\
 \mbox{and}\quad  |x^{\eps*}-x_j^{\eps*}-\tau(v_{k+1}^{\eps*}-v_j^{\eps*})| &\geq \eps_0/2\,.
 \end{aligned}  $$

$$ \begin{aligned} \cN^*( \bar x_j - \bar x_k,\bar v_j,\rho) (v_1) :=\big\{ (\nu ,v_2 )\in {\mathbf S}_1^{d-1}\times  B_R  \,/\, & (v_2-v_1) \cdot \nu > \eta \, ,  \\
&   v^*_1\in w+K(y,\rho) \hbox{ or }  v^*_2 \in w+K(y,\rho) \big\}\, 
\end{aligned}$$
Lemma \ref{geometric-lem3} bounds from the above the size of the set ${\mathcal N}^*(( \bar x_j - \bar x_k,\bar v_j,\rho)$ of all $(\nu,v_{k+1})\in  ({\mathbf S}_{1}^d \times B_R) \setminus C(\overline Z_k)$ such that 
% Now let us prove that the condition that $ v_k^{\eps*}, v_{k+1}^{\eps*} \in \bar v_j+K(\bar x_j -\bar x_k, 6CRa/\eps_0+6CR\eps_0/\delta) \cap B_R$ can be expressed  by a condition on  the post-collisional velocity $v_{k+1}$ and   the   angle~$\nu$ only.   This is made  possible thanks to Lemma~\ref{geometric-lem3}  according to which 
%\begin{equation}\label{defNZk}
$v_k^{\eps*}$ or $v_{k+1}^{\eps*}$ belongs to $\bar v_j+K(\bar x_j -\bar x_k, \rho).$ We let $\rho = 12Ra/\eps_0+12R\eps_0/\delta,$ and define
%) \Longrightarrow  (\nu,  v_{k+1}) \in \cN(\bar z_j,\bar z_k) \, ,
% \end{equation}
%with
% $$| \cN(\bar z_j,\bar z_k)| \leq C({\Phi,R,\eta})   \left( {a\over  \eps_0}+{ \eps_0\over \delta }\right)^{d-1}\,.$$
% 
%We therefore define~
$$\displaystyle \cM^{+} (\overline Z_k):= \bigcup_{j \leq k-1}  \cN^*(\bar x_j - \bar x_k,\bar v_j,\rho)$$ and $$
{\mathcal B}_k^+(\overline Z_k):= C(\overline Z_k) \cup \big( {\mathbf S}_1 ^{d-1} \times  \cM^{+} (\overline Z_k)  \big) \, ,
$$
where the set $C(\overline Z_k)$ is introduced in \eqref{defcone}. 
By Lemma \ref{geometric-lem3},
$$
\Big |{\mathcal B}_k^+(\overline Z_k) \Big | \leq   C ( R) \eta^{d-1} + C(\Phi,\eta,R) \big({a\over\eps_0}  +  {\eps_0\over\delta} \big)^{d-1}
$$
and~(\ref{taugeq0postcoll}) and~(\ref{taugeqdelta2postcoll}) hold as soon as~$(\nu,v) \notin {\mathcal B}_k^+(\overline Z_k)$.
 The proposition is proved.\qed
  
  Note that, in order to prove that pathological sets have vanishing measure as $\eps\to 0$, we have to choose~$\eta$ small enough, and then $a$ and $\eps_0$ even smaller in order that (\ref{sizeofparameters}) is satisfied and that (\ref{pathological-size}) is small.
  Note that, if we want to get a rate of convergence, we need to have more precise  bounds on the cross-section $b$ in terms of the truncation parameters $R$ and $\eta$.
  
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \section{Truncation of  the Boltzmann and BBGKY pseudo-trajectories}\label{truncationBB}
 In this paragraph we show that the previous geometrical result may be used to define approximate Boltzmann and BBGKY observables, corresponding to non pathological pseudo-trajectories. We then expect to be able to compare these approximate observables, which will be done in the next chapter.
 
%  The first step consists in preparing the initial configuration~$Z_s$ so that it is a good configuration. Then we show in Paragraph~\ref{approxboltzmann} 
% that the Boltzmann pseudo-trajectory may be used as a reference trajectory to apply Proposition~\ref{geometric-prop}, and  we truncate accordingly the  Boltzmann functional outside the bad phase-space sets defined in that proposition. The truncation of the BBGKY functional is carried out in   Paragraph~\ref{approxbbgky}.
% 
 
 
 
  \subsection{Initialization}\label{initialization}
 The first step consists in preparing the initial configuration~$Z_s$ so that it is a good configuration. We define
$$
\Delta_s (\eps_0):= \Big \{Z_s \in \R^{ds} \times B_R^s \, / \, \inf_{1 \leq \ell  < j \leq s}   |x_\ell-x_j| \geq \e_0 \Big \} \, ,
$$
and we shall  assume from now on that~$ Z_s $ belongs to~$ \Delta_s (\eps_0)$.  We also define for convenience
$$
\Delta_s^X (\eps_0):= \Big \{X_s \in \R^{ds}   \, / \, \inf_{1 \leq \ell  < j \leq s}   |x_\ell-x_j| \geq \e_0 \Big \} \, .
$$

 \begin{prop}\label{straightHs}
 For all~$X_s \in\Delta_s^X (\eps_0) $, there is a subset~${\mathcal M}_s (X_s)$ of~$\R^{ds}$ such that
 $$
\big |{\mathcal M}_s (X_s) \big |\leq C(R,s) \left(  \Big ({\eps\over\eps_0}\Big)^{d-1} + \Big ({\eps_0\over\delta}\Big)^{d-1}  \right) \,,
 $$
 and defining $\displaystyle
 {\mathcal P}_s := \Big\{
 Z_s \in \Delta_s  (\eps_0) \, / \, V_s \in {\mathcal M}_s (X_s)
 \Big\}  $,
 then \begin{equation}\label{goodinitialization}
 \begin{aligned}
 \forall \tau \geq 0 \,     , \quad    \indc_{ {\mathcal P}_s}\circ  {\bf H}_s(\tau) &  \equiv \indc_{ {\mathcal P}_s} \circ{\bf S}_s(\tau) \\
  \forall \tau \geq \delta  \, , \quad   \indc_{ {\mathcal P}_s} \circ {\bf S}_s(\tau) &  \equiv  \indc_{ {\mathcal P}_s} \circ {\bf S}_s(\tau) \circ  \indc_{ \cG_s(\eps_0)} \, .
   \end{aligned}
 \end{equation}
 denoting abusively by $\indc_A$ the operator of multiplication by the indicator of $A$.
\end{prop}
\begin{proof}
The proof is very similar to the arguments of the previous paragraph. For any~$Z_s$ in~$\Delta_s (\eps_0)$, we apply Lemma~\ref{geometric-lem1} which   shows that  outside a   small measure set~${\mathcal M}_s (X_s)\subset \R^{ds}$   of velocities~$(v_1,\dots,v_s)$, with
$$
|\cM_{s}(X_s) |\leq C (R) C^2_s \left({\eps\over\eps_0}+{\eps_0\over\delta}\right)^{d-1} \, ,
$$
 the backward nonlinear flow is actually the free flow and the particles remain at a distance larger than~$\eps$ to one  another for all times:
  $$ \forall \tau>0, \quad \forall \ell\neq \ell' \in \{1,\dots , s\} \, ,\quad |(x_ \ell-v_ \ell \tau)-(x_{\ell'} - v_{\ell'} \tau)| >\eps \, ,$$
and that
$$
 \forall \tau\geq\delta, \quad \forall \ell\neq \ell' \in \{1,\dots , s\} \, ,\quad |(x_ \ell-v_ \ell \tau)-(x_{\ell'} - v_{\ell'} \tau)| \geq \eps_0  \, .
$$
By construction, $\cM_s(X_s)$ depends continuously on $X_s$. Therefore, defining~$ {\mathcal P}_s := \{Z_s \in \Delta_s (\eps_0) \, / \, V_{s}  \notin  \cM_{s} (X_s)  \}$ gives the result. \end{proof}


% In the following we define with the notation of the proof of Proposition~\ref{straightHs},
%  $$
%   \forall X_s \in  \Delta_s^X (\eps_0) \, , \quad  {\mathcal P}^V_s :=    B_R^s \setminus \cM_{s}  (X_s )   $$
%     so that\label{defPsV}
%     $$
%     {\mathcal P}_s := \Big\{Z_s \in \Delta_s (\eps_0) \, / \, V_{s}  \in       {\mathcal P}^V_s \Big\} \, .
%     $$

 \subsection{Approximation of the Boltzmann functional}\label{approxboltzmann}
 We recall  that we consider a family of initial data~$F_{0} = (f_0^{(s)})$ satisfying
  $$
    \Nt{   F_{0} }_{0,\beta_0,\mu_0} = \sup_{s\in \N} \sup_{Z_s}\big( \exp(\beta_0 E (Z_s) +\mu_0 s)   f_{0}^{(s)}(Z_s) \big)<+\infty
$$
and after the reductions of Chapter~\ref{convergence}, the observable we are interested in is the following:
 \begin{equation} \label{elementary} 
   \begin{aligned}
    I^{0, R,\delta}_{s,n}   (t,J,M)(X_s) := \int  \varphi_s(V_s) \int_{{\mathcal T}_{n,\delta}(t) }   &{\bf S}_s(t-t_1) {\mathcal C}_{s,s+1}^{0,j_1,m_1} {\bf S}_{s+1}(t_1-t_2) {\mathcal C}^{0,j_2,m_2}_{s+1, s+2}\\
   &\dots   {\bf S}_{s+n}(t_n- t_{n+1})  \indc_{|E_0(Z_{s+n})|\leq R^2} f^{(s+n)}_{0}   dT_n dV_s\, ,
   \end{aligned}
    \end{equation}
By Proposition \ref{straightHs}, up to an error term of order $C(R ) s^2 \left({\eps/\eps_0}+{\eps_0/\delta}\right)^{d-1}$, we can assume that the initial configuration $Z_s$ is a good configuration, meaning that 
$$
\begin{aligned}
  I^{0,R,\delta}_{s,n}(t,J,M )(X_s)  = \int_{B_R \setminus \cM_s(X_s)}  \varphi_s(V_s) &\int_{{\mathcal T}_{n,\delta}(t) }   {\bf S}_s(t-t_1) {\mathcal C}_{s,s+1}^{0,j_1,m_1} {\bf S}_{s+1}(t_1-t_2) {\mathcal C}^{0,j_2,m_2}_{s+1, s+2}\\
&  \dots {\mathcal C}^{0,j_n,m_n}_{s+n-1 , s+n}  {\bf S}_{s+n}(t_n- t_{n+1}) \indc_{|E_0(Z_{s+n})|\leq R^2}   f^{(s+n)}_{0}   \,dT_ndV_s \\
+ O\Big(C(R ) s^2 &\left({\eps\over \eps_0}+{\eps_0\over \delta}\right)^{d-1} \Big) \, ,
\end{aligned}
$$
where
$$
 \begin{aligned}\big({\mathcal C}^{0,-,m}_{s,s+1}   f^{(s+1)}  \big)(Z_s)
 &= \int_{ {\bf S}_{1}^{d-1} \times \R^d}  ((v_{s+1}-v_m)\cdot \nu_{s+1})_-  f^{(s+1)}  (Z_s, x_m, v_{s+1}) \, d\nu_{s+1} dv_{s+1} \quad \mbox{and}
\\
\big({\mathcal C}^{0,+,m}_{s,s+1}   f^{(s+1)}  \big)(Z_s)
& =  \int_{ {\bf S}_{1}^{d-1} \times \R^d} \! \! \! \! \! 
 ((v_{s+1}-v_m)\cdot \nu_{s+1})_+   f^{(s+1)}  ( z_1, \dots ,x_m, v^*_m,\dots ,z_s, x_m, v^*_{s+1}) \,d\nu _{s+1}dv_{s+1}\, .
\end{aligned}
$$

 Now let us introduce some notation which we shall be using constantly from now on: 
given~$Z_s \in \Delta_s (\eps_0)$, we call~$Z_s^0(\tau)$ the position of the backward free flow initiated from~$Z_s$, at time~$t_1\leq \tau \leq t$. Then given~$j_1 \in \{+,-\}$, $m_1 \in [1,s]$, a deflection angle~$\omega_{s+1}$ and a velocity~$v_{s+1} $ we call~$Z_{s+1}^0(\tau )$ the   position at time~$   t_2 \leq \tau < t_1$ of the Boltzmann pseudo-trajectory initiated by the adjunction of the particle~$(\nu_{s+1},v_{s+1})$ to the particle~$z_{m_1}^0(t_1)$ (which is simply free-flow in the pre-collisional case~$j_1 = -$, and free-flow after scattering of particles~$z_{m_1}^0(t_1)$ and~$(\nu_{s+1},v_{s+1})$ in the post-collisional case~$j_1 = +$). 

Similarly by induction given~$Z_s \in \Delta_s (\eps_0)$, $T, J$ and~$M$ we denote for each~$1 \leq k \leq n$ by~$Z_{s+k}^0(\tau )$ the position at time~$ t_{k+1} \leq   \tau < t_k $ of the pseudo-trajectory initiated by the adjunction of the particle~$(\nu_{s+k},v_{s+k})$ to the particle~$z_{m_k}^0(t_k)$ (which is simply free-flow in the pre-collisional case~$j_k = -$, and free-flow after scattering of particles~$z_{m_k}^0(t_k)$ and~$(\nu_{s+k},v_{s+k})$ in the post-collisional case~$j_k= +$). 

Notice that~$\tau \mapsto~Z_{s+k}^0(\tau )$ is pointwise right-continuous on~$[0,t_k]$.
 
With this notation, the functional~$   I^{0,R,\delta}_{s,n}$ may be reformulated as 
 $$
  \begin{aligned}
     I^{0,R,\delta}_{s,n} (t,J,M)(X_s)&   =  \int_{B_R \setminus \cM_s(X_s)} dV_s  \varphi_s(V_s) 
     \int_{{\mathcal T}_{n,\delta}(t) }  dT_n
  \int_{{\mathbf S}^{d-1}_{1} \times B_R} \!  \!  \!  \!  \!  d\nu_{s+1} dv_{s+1}
  ((v_{s+1} - v_{m_1}^0(t_1)\cdot \nu_{s+1} )_+ \\
       &\dots    \int_{{\mathbf S}^{d-1}_{1} \times B_R}   \!  \!  \!  \!  \! d\nu_{s+n} dv_{s+n}
  ((v_{s+n} - v_{m_n}^0(t_n)\cdot \nu_{s+n} )_+  \indc_{E_0(Z_{s+n}^0 (0))\leq R^2}    f^{(s+n)}_{0}   (Z_{s+n}^0 (0)) \\
  &+ O\Big(C(R ) s^2 \left({\eps\over \eps_0}+{\eps_0\over \delta}\right)^{d-1} \Big) \, .
   \end{aligned}
  $$
  
  Let $ a,\eps_0,\eta\ll 1$  be  such that
$$
 a \ll \eps_0 \ll \eta \delta \, .
$$
According to  Proposition~\ref{geometric-prop},  for any good configuration~$\overline Z_{s+k-1} \in \R^{2d(s+k-1)}$, we can define a set  $$
 ^c{} {\mathcal B}_{s+k-1} (\overline Z_{s+k-1}):=\big( {\mathbf S}^{d-1}_{1} \times B_R \big)\setminus {\mathcal B}_{s+k-1} (\overline Z_{s+k-1} )\, ,
$$
such that good configurations $Z_{s+k-1}=(X_{s+k-1}, \overline V_{s+k-1})$ with $|X_{s+k-1}-\overline X_{s+k-1}|\leq Ca$  are stable by adjunction of a collisional particle $(\nu_{k+s}, v_{k+s}) \in ^c{} {\mathcal B}_{s+k-1}^ (\overline Z_{s+k-1})$.


We further notice that
thanks to  Remark~\ref{betterresult}, if the adjoined pair~$(\nu_{s+k},v _{s+k})$ belongs to the set~$ ^c{} {\mathcal B}_{s+k-1}(  Z_{s+k-1}^0(t_k))$ with~$ Z_{s+k-1}^0(t_k) \in \cG_{s+k-1}(\eps_0)$, then~$Z_{s+k}^0(t_{k+1}) $ belongs to~$\cG_{s+k }(\eps_0)$.


As a consequence we may define recursively the approximate Boltzmann functional
 \begin{equation}\label{boltzmannfunctionalapprox}
  \begin{aligned}
 J^{0,R,\delta}_{s,n} (t,J,M)(X_s)   & =  \int_{B_R \setminus \cM_s(X_s)} dV_s  \varphi_s(V_s) 
     \int_{{\mathcal T}_{n,\delta}(t) }  dT_n\\
  &   \quad 
    \int_{^c{} {\mathcal B}_{s} (  Z_s^0(t_1))} \!  \!  \!  \!  \!  d\nu_{s+1} dv_{s+1}
  (v_{s+1} - v_{m_1}^0(t_1)\cdot \nu_{s+1} )_{j_1} \\
& \qquad       \dots    \int_{^c{} {\mathcal B}_{s+n-1}i (  Z_{s+n-1}^0(t_n))}   \!  \!  \!  \!  \! d\nu_{s+n} dv_{s+n}
  (v_{s+n} - v_{m_n}^0(t_n)\cdot \nu_{s+n} )_{j_n} \\
  & \qquad\qquad\times \indc_{E_0(Z_{s+n}^0 (0))\leq R^2}    f^{(s+n)}_{0}   (Z_{s+n}^0 (0))  \, .
   \end{aligned}
  \end{equation}
The following result is an immediate consequence of Proposition~\ref{geometric-prop} 
\begin{prop}\label{lastapproxb}
  Let $a,\eps_0,\eta\ll 1$  satisfying {\rm(\ref{sizeofparameters})}.
  Then, 
  $$
\begin{aligned}
&\Big| \1_{\Delta_s (\eps_0)} \big (   I_{s,n}^{0,R,\delta}-   J_{s,n}^{0,R,\delta } \big) (t,J,M )   \Big|  \leq (s+n)^2 \left( C(R ) \eta^{d-1} + C(R,\Phi,\eta) \Big(
  \frac{a}{\eps_0} +  \frac{\eps_0}{\delta} 
\Big)^{d-1}\right)  \Nt{   F_{0}}_{0,\beta_0,\mu_0} \, .
\end{aligned}
$$
\end{prop}
  
 \subsection{Approximation of the BBGKY functional}\label{approxbbgky}
We recall that after the reductions of Chapter~\ref{convergence}, the functional we are interested in is
 $$
 \begin{aligned}
I_{s,n} ^{R,\delta}  (t,J,M)(X_s) := \int  \varphi_s(V_s) \int_{{\mathcal T}_{n,\delta}(t) }   &{\bf H}_s(t-t_1){\mathcal C}_{s,s+1}^{j_1,m_1} {\bf H}_{s+1}(t_1-t_2) {\mathcal C}^{j_2,m_2}_{s+1, s+2}\\
   &\dots{\mathcal C}^{j_n,m_n}_{s+n-1 , s+n}  {\bf H}_{s+n}(t_n- t_{n+1})\indc_{|E_\eps(Z_{s+n})|\leq R^2} \widetilde f^{(s+n)}_{N,0}   dT_n dV_s\, ,
    \end{aligned}
$$ 
where~$\widetilde  F_{N,0} = (\widetilde f_{N,0}^{(s)})_{1 \leq s \leq N}$ satisfies
  $$
    \Nt{ \widetilde  F_{N,0}  }_{\eps,\beta_0,\mu_0} = \sup_{s\in \N} \sup_{Z_s}\big( \exp(\beta_0 E_\eps (Z_s) +\mu_0 s) \widetilde  f_{N,0}^{(s)}(Z_s) \big)<+\infty \, .
$$
Thanks to Proposition~\ref{initialization}, we have
$$
 \begin{aligned}
        I^{R,\delta}_{s,n}  (t,J,M)(X_s) = \int _{B_R \setminus \cM_s(X_s)} \varphi_s(V_s) \int_{{\mathcal T}_{n,\delta}(t) }   &{ \bf S}_s(t-t_1) \indc_{{\mathcal G}_s(\eps_0)}{\mathcal C}_{s,s+1}^{j_1,m_1} {\bf H}_{s+1}(t_1-t_2) {\mathcal C}^{j_2,m_2}_{s+1, s+2}\\
   &\dots {\mathcal C}^{ j_n,m_n}_{s+n-1 , s+n}  {\bf H}_{s+n}(t_n- t_{n+1})  \indc_{E_\eps(Z_{s+n}(0))\leq R^2}     \widetilde f_{N,0}^{(s+n)}  dT_n  dV_s\\
    + O\Big(C(R ) s^2 &\left({\eps\over \eps_0}+{\eps_0\over \delta}\right)^{d-1} \Big) \, .
   \end{aligned}
$$

Then using the notation introduced in the previous paragraph for the Boltzmann pseudo-trajectory, let us define
 the approximate functionals
$$
 \begin{aligned}
       J_{s,n} ^{R,\delta} (t,J,M)(X_s) := \int _{B_R \setminus \cM_s(X_s)} \varphi_s(V_s) \int_{{\mathcal T}_{n,\delta}(t) }   { \bf S}_s(t-t_1) \indc_{{\mathcal G}_s(\eps_0)}\widetilde {\mathcal C}_{s,s+1}^{j_1,m_1} {\bf H}_{s+1}(t_1-t_2) \\
   \dots \widetilde{\mathcal C}^{ j_n,m_n}_{s+n-1 , s+n}  {\bf H}_{s+n}(t_n- t_{n+1}) \indc_{E_\eps(Z_{s+n}(0))\leq R^2}      \widetilde f_0^{(s+n)}  dT_n  dV_s \, ,
   \end{aligned}
$$
where
$$
 \begin{aligned}
\big(\widetilde {\mathcal C}_{s+k-1,s+k}^{-,m_k} g^{(s+k)} \big) (Z_{s+k-1})  :=   (N- s-k+1) \eps^{d-1} 
 \int_{  ^c{} {\mathcal B}_{s+k-1}  (  Z_{s+k-1}^0(t_k))
}   (\nu_{s+k}   \cdot ( v_{s+k}  - v_{m_k}(t_k)))_-  \\ 
   \times  {} g^{(s+k)}  (\cdot, x_{m_k} (t_k)+  \eps \nu_{s+k}  ,v_{s+k}(t_k))  \prodetage{1 \leq j \leq s +k-1}{j \neq m_k} \indc_{|(x_j-x_{m_k})(t_k)-\eps \nu_{s+k}| \geq \eps}   \, d\nu_{s+k}  dv_{s+k} \\
   \big(\widetilde {\mathcal C}_{s+k-1,s+k}^{+,m_k} g^{(s+k)} \big) (Z_{s+k-1})  :=   (N- s-k+1) \eps^{d-1} 
 \int_{  ^c{} {\mathcal B}_{s+k-1}  (  Z_{s+k-1}^0(t_k))
}   (\nu_{s+k}   \cdot ( v_{s+k}  - v_{m_k}(t_k)))_+  \\ 
   \times  {} g^{(s+k)}  (\dots,x_{m_k}^*, v_{m_k}^*, \dots , x^*_{s+k}   ,v_{s+k}^*)  \prodetage{1 \leq j \leq s +k-1}{j \neq m_k} \indc_{|(x_j-x_{m_k})(t_k)-\eps \nu_{s+k}| \geq \eps}   \, d\nu_{s+k}  dv_{s+k} \, .
\end{aligned}
$$
denoting as previously by $(x_{m_k}^*, v^*_{m_k}, x^*_{s+k}   ,v_{s+k}^*)$ the pre-image of $ (x_{m_k}, v_{m_k}(t_k), x_{m_k} (t_k)+  \eps \nu_{s+k}  ,v_{s+k}(t_k))$ by the scattering $\sigma_\eps$.


As in the Boltzmann case described above, the following result is an immediate consequence of Proposition~\ref{geometric-prop}.
\begin{prop}\label{lastapproxbbgky}
 Let $a,\eps_0,\eta\ll 1$  satisfying {\rm(\ref{sizeofparameters})}.
  Then, for $\eps$ sufficiently small,
  $$
\begin{aligned}
&\Big| \1_{\Delta_s (\eps_0)} \big (   I_{s,n}^{R,\delta}-   J_{s,n}^{R,\delta } \big) (t,J,M )   \Big|  \leq (s+n)^2 \left( C(R ) \eta^{d-1} + C(R,\Phi,\eta) \Big(
  \frac{a}{\eps_0} +  \frac{\eps_0}{\delta} 
\Big)^{d-1}\right)  \Nt{  \widetilde F_{N,0}}_{\eps,\beta_0,\mu_0} \, .
\end{aligned}
$$
\end{prop}

   The functional~$J_{s,n} ^{R,\delta}$ can be written in terms of pseudo-trajectories, as in~(\ref{boltzmannfunctionalapprox}).  Let us therefore  introduce some notation which we shall be using constantly from now on: 
given~$Z_s \in \Delta_s (\eps_0)$, we call~$Z_s^0(\tau)$ the position of the backward free flow initiated from~$Z_s$, at time~$t_1 \leq \tau \leq t$. Then given~$j_1 \in \{+,-\}$, $m_1 \in [1,s]$, an angle~$\nu_{s+1}$ (or equivalently a position~$x_{s+1} = x_{m_1}^0(t_1) + \eps \nu_{s+1}$) and a velocity~$v_{s+1} $ we call~$Z^\eps_{s+1}(\tau)$ the   position at time~$ t_2 \leq \tau < t_1$ of the BBGKY pseudo-trajectory initiated by the adjunction of the particle~$z_{s+1}$ to the particle~$z_{m_1}^0(t_1)$. 

Similarly by induction given~$Z_s \in \Delta_s (\eps_0)$, $T, J$ and~$M$ we denote for each~$1 \leq k \leq n$ by~$Z^\eps_{s+k}(\tau )$ the position at time~$  t_{k+1} \leq \tau< t_k $ of the BBGKY pseudo-trajectory initiated by the adjunction of the particle~$z_{s+k}$ to the particle~$z_{m_k}(t_k)$. 
We have
\begin{equation}\label{firstbbgkypseudotraj}
 \begin{aligned}
  & J_{s,n} ^{R,\delta} (t,J,M)(X_s) = \frac{(N-s)! }{(N- s-n)!}\eps^{n(d-1)} \int_{B_R \setminus \cM_s(X_s)} dV_s \varphi_s(V_s) \int_{{\mathcal T}_{n,\delta}(t) }   dT_n    \\
&\quad \int_{  ^c{} {\mathcal B}_{s}  (  Z_{s}^0(t_1))
}   d\nu_{s+1}  dv_{s+1} \,   (\nu_{s+1}   \cdot ( v_{s+1}  - v_{m_1}(t_1)))_{j_1}  \prodetage{1 \leq j \leq s}{j \neq m_1} \indc_{|(x_j-x_{m_1})(t_1)-\eps \nu_{s+1}| \geq \eps}   \\ 
 & \quad \dots  \int_{  ^c{} {\mathcal B}^{j_n}_{s+n-1}  (  Z_{s+n-1}^0(t_n))
}  d\nu_{s+n}  dv_{s+n}  \, (\nu_{s+n}   \cdot ( v_{s+n}  - v_{m_n}(t_n)))_{j_n}   \\ 
  &\quad \times   \prodetage{1 \leq j \leq s +n-1}{j \neq m_n} \indc_{|(x_j-x_{m_n})(t_n)-\eps \nu_{s+n}   | \geq \eps}  
 \indc_{E_\eps(Z_{s+n}(0))\leq R^2}      \widetilde f_{N,0}^{(s+n)} (Z^\eps_{s+n}(0))   \, .
\end{aligned}
\end{equation}

Thanks to Propositions~\ref{lastapproxb} and~\ref{lastapproxbbgky} the proof of Theorem~\ref{main-thm}
 reduces to the proof of the convergence to zero of~$ J^{R,\delta}_{s,n}-  J^{0,R,\delta}_{s,n}$. This is the object of the next chapter.
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
